Fast and Certifiable Trajectory Optimization

We propose semidefinite trajectory optimization (STROM), a framework that computes fast and certifiably optimal solutions for nonconvex trajectory optimization problems defined by polynomial objectives and constraints. STROM employs sparse second-order Lasserre's hierarchy to generate semidefinite program (SDP) relaxations of trajectory optimization. Different from existing tools (e.g., YALMIP and SOSTOOLS in Matlab), STROM generates chain-like multiple-block SDPs with only positive semidefinite (PSD) variables. Moreover, STROM does so two orders of magnitude faster. Underpinning STROM is cuADMM, the first ADMM-based SDP solver implemented in CUDA and runs in GPUs (with C/C++ extension). cuADMM builds upon the symmetric Gauss-Seidel ADMM algorithm and leverages GPU parallelization to speedup solving sparse linear systems and projecting onto PSD cones. In five trajectory optimization problems (inverted pendulum, cart-pole, vehicle landing, flying robot, and car back-in), cuADMM computes optimal trajectories (with certified suboptimality below 1%) in minutes (when other solvers take hours or run out of memory) and seconds (when others take minutes). Further, when warmstarted by data-driven initialization in the inverted pendulum problem, cuADMM delivers real-time performance: providing certifiably optimal trajectories in 0.66 seconds despite the SDP has 49,500 variables and 47,351 constraints.

==> figs/exp-cr-compare/fig.tex <==
%!TEX root = ../../main.tex

\begin{figure}[htbp]
    \label{fig:exp:cr:compare}
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.7\columnwidth]{figs/exp-cr-compare/legend.png}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-cr-compare/kkt.png}
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-cr-compare/subopt_gap.png}
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-cr-compare/time.png}
            \end{minipage}

            \begin{minipage}{0.22\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-cr-compare/iter_num.png}
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{Four SDP solvers' performance comparison in the car back-in case.}
\end{figure}

==> figs/exp-cr-demos/fig.tex <==
%!TEX root = ../../main.tex

\begin{figure}
    \label{fig:exp:cr:demos}
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \begin{minipage}{0.25\textwidth}
                \centering
                \vspace{0.5mm}
                \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=6_ry=3_th=0/traj_fea.pdf}
                (a)
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=-1_ry=2_th=0/traj_fea.pdf}
                (b)
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \vspace{0.5mm}
                \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=0_ry=0_th=-1/traj_fea.pdf}
                (c)
            \end{minipage}
        \end{tabular}
    \end{minipage}

    % \begin{minipage}{\textwidth}
    %     \centering
    %     \begin{tabular}{ccc}
    %         \begin{minipage}{0.33\textwidth}
    %             \centering
    %             \vspace{4.5mm}
    %             \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=-5_ry=4_th=-2/traj_fea.pdf}
    %             (d)
    %         \end{minipage}

    %         \begin{minipage}{0.33\textwidth}
    %             \centering
    %             \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=-5_ry=4_th=1/traj_fea.pdf}
    %             (e)
    %         \end{minipage}

    %         \begin{minipage}{0.33\textwidth}
    %             \centering
    %             \vspace{5.5mm}
    %             \includegraphics[width=\columnwidth]{figs/exp-cr-demos/N=30_freq=4_vmax=4_wmax=1_rx=-1_ry=4_th=3/traj_fea.pdf}
    %             (f)
    %         \end{minipage}
    %     \end{tabular}
    % \end{minipage}

    \caption{Global optimal motions for the car back-in problem.}
    
\end{figure}

==> figs/exp-p-boxplot/fig.tex <==
%!TEX root = ../../main.tex

\begin{figure}[htbp]
    \label{fig:exp:p:boxplot}
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.7\columnwidth]{figs/exp-p-boxplot/legend.png}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{cccc}
            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-boxplot/kkt.png}
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-boxplot/subopt_gap.png}
            \end{minipage}

            \begin{minipage}{0.25\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-boxplot/time.png}
            \end{minipage}

            \begin{minipage}{0.22\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-boxplot/iter_num.png}
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{Five SDP solvers' performance comparison in the pendulum case. From left to right: max KKT residual $\eta$; suboptimality gap $\xi$; total time cost; iteration number for first-order solvers.}
\end{figure}

==> figs/exp-p-mpc-knn/fig.tex <==
%!TEX root = ../../main.tex

\begin{figure}[htbp]
    \label{fig:exp:p:mpc-knn}
    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \begin{minipage}{0.33\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/u_realtraj.png}
            \end{minipage}

            \begin{minipage}{0.33\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/th_realtraj.png}
            \end{minipage}

            \begin{minipage}{0.33\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/dth_realtraj.png}
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \begin{minipage}{\textwidth}
        \centering
        \begin{tabular}{ccc}
            \begin{minipage}{0.35\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/subopt_gap.png}
            \end{minipage}

            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/time.png}
            \end{minipage}

            \begin{minipage}{0.32\textwidth}
                \centering
                \includegraphics[width=\columnwidth]{figs/exp-p-mpc-knn/iter_num.png}
            \end{minipage}
        \end{tabular}
    \end{minipage}

    \caption{Simulated MPC with kNN warm start in the pendulum case.}
\end{figure}

==> sections/cartpole.tex <==
%!TEX root = ../../main.tex

\subsection{Cart-Pole}
\label{subsec:exp:ca}

For cart-pole, the continuous-time state is $a, \dot{a}, \theta, \dot{\theta}$, where $a$ is the cart's position and $\theta$ is the pole's angle. With the help of the Lie group variational integrator, we can discretize the two-body dynamics as quadratic polynomial constraints. See details in \S\ref{app:subsec:exp:ca}. Figure~\ref{fig:exp:ca:demos-plots} shows three globally optimal trajectories for cart-pole. Figure~\ref{fig:exp:ca:mpc} shows the results of simulated MPC. Starting from $a_0 = 0, \dot{a}_0 = 0, \theta_0 = 0.1, \dot{\theta}_0 = 0$, we want to achieve $a = 0, \dot{a} = 0, \theta = \pi, \dot{\theta} = 0$. We take the last step's optimal SDP
solution as the next step's initial guess. Our certifiable controller can stabilize the cart-pole system.
\input{figs/exp-ca-demos-plots/fig.tex}
\input{figs/exp-ca-mpc/fig.tex}
 


==> sections/vehicle-landing.tex <==
%!TEX root = ../../main.tex

\subsection{Vehicle Landing}
\label{subsec:exp:vl}

We want to land a planer vehicle with two boosters in this experiment. The vehicle has six continuous-time states: 2-D position $(x, y)$, 2-D velocity $(\dot{x}, \dot{y})$, angular position $\theta$ and velocity $\dot{\theta}$. The discretization procedure is similar to the pendulum case. Please refer to \S\ref{app:subsec:exp:vl}. Figure~\ref{fig:exp:vl:demos-plots} shows three globally optimal trajectories.
\input{figs/exp-vl-demos-plots/fig.tex}


==> tables/hyper_params.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:hyper-params}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & $d_x$ & $d_u$ & $\text{deg}_{\max}$ & $N$ & $\text{size}(M)$ & $\#M$ & $\text{size}(L)$ & $\#L$ & $m_{\text{SDP}}$ & $\log_{10}\xi$ \\
        \hline 
        Inverted Pendulum & $4$ & $1$ & $2$ & $30$ & $55$ & $30$ & $10$ & $60$ & $47351$ & $\bm{-2.58}$ ($\bm{-2.93}$) \\
        \hline 
        Cart-Pole & $5$ & $1$ & $2$ & $30$ & $105$ & $30$ & $14$ & $273$ & $168961$ & $\bm{-2.89}$ ($\bm{-2.98}$) \\
        \hline 
        Car Back-in & $4 (+3)$ & $4$ & $3$ & $30$  & $190$ & $30$ & $19$ & $659$ & $509141$ & $\bm{-1.87}$ ($\bm{-1.99}$) \\
        \hline 
        Vehicle Landing & $8$ & $2$ & $2$ & $50$ & $190$ & $50$ & $19$ & $499$ & $946326$ & $\bm{-2.47}$ ($\bm{-2.42}$) \\
        \hline 
        Flying Robot & $8$ & $4$ & $2$ & $60$ & $231$ & $60$ & $21$ & $659$ & $1595001$ & $\bm{-2.57}$ ($\bm{-2.49}$) \\
        \hline 
    \end{tabular}
    }

    \caption{Hyper-parameters and suboptimality gaps in five numerical experiments. Means (medians) are reported for suboptimality gaps from \cuadmm. In the car back-in case, $(+3)$ denotes the $(A,B,C)$ parameters in the separation line.}
\end{table}

==> tables/timing.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
    \label{tab:exp:gen:timing}
    \centering
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{} & \multicolumn{4}{c|}{Per-Iteration Cost} & \multicolumn{4}{c|}{Total Time} \\
        \cline{2-9}
        & \mosek & \cdcs & \sdpnal & \cuadmm & \mosek & \cdcs & \sdpnal & \cuadmm \\
        \hline 
        \multirow{2}{*}{Inverted Pendulum} & \multirow{2}{*}{$0.5$s} & \multirow{2}{*}{$11.1$ms} & \multirow{2}{*}{$59.1$ms} & \multirow{2}{*}{\textbf{$\bm{8.9}$ms}} & \multirow{2}{*}{$9.5$s} & \multirow{2}{*}{$110.3$s} & \multirow{2}{*}{$264.4$s} & $31.2$s ($14.6$s) \\
        \cline{9-9} 
        & & & & & & & & \textbf{$\bm{0.66}$s} (\textbf{$\bm{0.62}$s}) \\
        \hline
        Cart-Pole & $7.5$s & $147.1$ms & $588.2$ms & \textbf{$\bm{29.1}$ms} & \textbf{$\bm{112.0}$s} & $1471$s & $3671$s & $183.0$s ($173.1$s) \\
        \hline 
        Car Back-in & $778.1$s & $612.3$ms & $1.8$s & $\bm{44.8}$\textbf{ms} & $>5$h & $6123$s & $>5$h & \textbf{$\bm{431.5}$s} (\textbf{$\bm{536.8}$s})  \\
        \hline 
        Vehicle Landing & $1387$s & $1.0$s & $2.4$s & $\bm{118.3}$\textbf{ms} & $>5$h & $2.9$h & $>5$h &  \textbf{$\bm{919.2}$s} (\textbf{$\bm{1165}$s}) \\
        \hline 
        Flying Robot & - & $1.7$s & $6.2$s & $\bm{169.7}$\textbf{ms} & - & $>5$h & $>5$h & \textbf{$\bm{1648}$s} (\textbf{$\bm{2027}$s}) \\
        \hline 
    \end{tabular}
    }

    \caption{Per-interation costs and total time costs for different solvers across five experiments. For \cuadmm, we report the means (medians) of total time costs. The pendulum case lists total time costs with (upper) and without (lower) warm starts. For the flying robot case, \MOSEK runs out of 1TB memory.}
\end{table}
